NAS-X: Neural Adaptive Smoothing via Twisting

Sequential latent variable models (SLVMs) are essential tools in statistics and machine learning, with applications ranging from healthcare to neuroscience. As their flexibility increases, analytic inference and model learning can become challenging, necessitating approximate methods. Here we introduce neural adaptive smoothing via twisting (NAS-X), a method that extends reweighted wake-sleep (RWS) to the sequential setting by using smoothing sequential Monte Carlo (SMC) to estimate intractable posterior expectations. Combining RWS and smoothing SMC allows NAS-X to provide low-bias and low-variance gradient estimates, and fit both discrete and continuous latent variable models. We illustrate the theoretical advantages of NAS-X over previous methods and explore these advantages empirically in a variety of tasks, including a challenging application to mechanistic models of neuronal dynamics. These experiments show that NAS-X substantially outperforms previous VI- and RWS-based methods in inference and model learning, achieving lower parameter error and tighter likelihood bounds.

==> figure_tex/lgssm/comparisons.tex <==
\begin{figure*}
    \centering
        \includegraphics[scale=0.465]{figures/lgssm/unified_fig_lgssm.pdf}
    \caption{\textbf{Comparison of NAS-X vs NASMC on Inference in LG-SSM.} 
    (\textbf{left}) Comparison of learned proposal means. (\textbf{middle}) Comparison of learned proposal variances. (\textbf{right}) Comparison of log-marginal likelihood bounds (lower is better). NAS-X's learned proposal captures the true posterior mean and variance and achieves tighter estimates of the log marginal likelihood.}
    \label{fig:exp:lgssm_full}
    \vspace{-5mm}
\end{figure*}


==> figure_tex/nascar/nascar_model_lrn.tex <==
\begin{figure*}[!ht]
    \centering
    \begin{subfigure}{\textwidth}
        \includegraphics[scale=0.45]{figures/nascar/nascar_qualitative_model_lrn_obs_var=1e-3.pdf}
        \vspace*{-0.5cm}        \label{fig:exp:nascar_lrn:qual_plot}
    \end{subfigure}%
    \caption{Model learning results for recurrent switching linear dynamical systems. \textbf{(a)} Comparison of learned dynamics and inferred latent states.}
    \label{fig:exp:nascar_model_lrn}
\end{figure*}



==> table_tex/hh_bounds.tex <==
\begin{table}[h]
\centering
\caption{BPF bound comparison}
\begin{tabular}{cc}
\toprule
\textbf{Method} & $\mathcal{L}_\mathrm{BPF}^{256}$ \\
\toprule
NAS-X & -660.7003 \\
SIXO & \textbf{-636.2579} \\
\toprule
\label{table:hh_model_bounds}
\end{tabular}
\end{table}

==> table_tex/hh_features.tex <==
\begin{table}[h]
\centering
\caption{Comparison of Biophysical Features of Learned Models}
\begin{tabular}{ccccc}
\toprule
Method  & Num spikes & Avg Volt & Voltage Std & Cross Corr \\
\toprule
NAS-X & $\mathbf{0.755 \pm 0.15}$ & ${0.0358 \pm 0.0012}$ & 
${2.8142 \pm 0.088}$ & $\mathbf{6258.0022 \pm 11.06}$ \\
SIXO & $1.88 \pm 0.411$  & $\mathbf{0.0340 \pm 0.0034}$ & $\mathbf{2.3543 \pm 0.1957}$ & ${6055.87 \pm 21.98}$
\toprule
\end{tabular}
\label{table:hh_model_feature}
\end{table}

